The era of the ARG: an empiricist's guide to ancestral recombination graphs

In the presence of recombination, the evolutionary relationships between a set of sampled genomes cannot be described by a single genealogical tree. Instead, the genomes are related by a complex, interwoven collection of genealogies formalized in a structure called an ancestral recombination graph (ARG). An ARG extensively encodes the ancestry of the genome(s) and thus is replete with valuable information for addressing diverse questions in evolutionary biology. Despite its potential utility, technological and methodological limitations, along with a lack of approachable literature, have severely restricted awareness and application of ARGs in empirical evolution research. Excitingly, recent progress in ARG reconstruction and simulation have made ARG-based approaches feasible for many questions and systems. In this review, we provide an accessible introduction and exploration of ARGs, survey recent methodological breakthroughs, and describe the potential for ARGs to further existing goals and open avenues of inquiry that were previously inaccessible in evolutionary genomics. Through this discussion, we aim to more widely disseminate the promise of ARGs in evolutionary genomics and encourage the broader development and adoption of ARG-based inference.

==> figures/tex_files/arg_review_main_figure.tex <==
%% FIGURE %%
%\begin{figure}[!ht]
\begin{figure}[ht!]
\renewcommand{\thefigure}{\arabic{figure}}


%\renewcommand{\thefigure}{\arabic{figure}S}
\includegraphics[width=\textwidth]
{figures/pdfs/arg_review_main_figure.pdf}\caption{\label{fig:arg_review_main_figure}Visual and tabular depictions of the ancestral recombination graph (ARG). More text.... I have a couple of uncertainties about things shown here, especially the annotations on the marginal trees.}
\label{arg_review_main_figure}
\end{figure}
%%%%

==> sections/0_highlights.tex <==
%%Research highlights
\begin{highlights}
\item Ancestral recombination graphs (ARGs) contain all knowable information regarding relatedness in the genome.

\item Technological and methodological limitations have hitherto rendered ARGs inaccessible for most evolutionary genomics research. However, recent breakthroughs in reconstruction and simulation of the ARG have made ARG-based inference increasingly achievable.

\item some other highlight (the highlights are collectively limited to 900 characters including spaces and should contain 3--5 statement)
\end{highlights}

==> sections/8_figures.tex <==
\section{Figures}

%%% FIG 1. STUDY OVERVIEW %%%
%%\input{figures/tex_files/arg_review_main_figure}
%\input{figures/tex_files/arg_review_main_figure_VersiongARG}


%%% FIG 2. TREE SEQUENCE FIG %%%
%%%\input{figures/tex_files/arg_review_main_figure}
%\input{figures/tex_files/arg_mutation_fig}

%%% FIG 3. AN ARG INTUITION %%%
%%%\input{figures/tex_files/arg_review_main_figure}
%\input{figures/tex_files/arg_intuition_sim_fig}



==> sections/NOTINCLUDED4_method_developments.tex <==
\section{Methodological progress related to ARGs}
\label{sec:methods}
Although there has been a longstanding interest in ARG inference and analysis since the concept's introduction, impressive innovations in ARG-based methods over the past $\sim$10 years, together with breakthroughs in genome sequencing, have accelerated the practical relevance of ARGs across diverse arenas of evolutionary biology and other fields like medical genomics. Below, we briefly survey this increasingly mature and user-friendly ecosystem of methods and software.

\subsection*{ARG reconstruction}
A growing arsenal of methods is being developed to infer ARGs from genomic data. \texttt{ARGweaver}, which was introduced in \citeyear{Rasmussen2014Genome-WideGraphs} by \citeauthor{Rasmussen2014Genome-WideGraphs}, represents a seminal achievement in ARG inference. \texttt{ARGweaver} and its extension (\texttt{ARGweaver-D}; \citealt{Hubisz2020MappingGraph}) leverage approximations of the coalescent [SMC or SMC' \citep{Marjoram2006FastSimulation}] and time discretization to simplify the space from which to sample candidate ARGs using Markov Chain Monte Carlo. These methods, along with other recent Bayesian approaches like \texttt{Arbores} \citep{Heine2018BridgingGraphs} and \texttt{ARGinfer} \citep{Mahmoudi2022BayesianGraphs} enable the rigorous treatment of ARG uncertainty via the incorporation of the ARG's posterior distribution into downstream analyses. One general limitation of these methods is that, due to computational requirements, they can only handle fairly modest sample sizes. For example, \texttt{ARGweaver} can consider between two to about 100 samples \citep{Hubisz2020InferenceARGweaver}.

Motivated by the extensive sequencing efforts in human genomics, several methods have been devised to accommodate large and complicated genomic datasets. For example, \texttt{ARG-Needle} \citep{Zhang2023Biobank-scaleTraits}, \texttt{tsinfer}/\texttt{tsdate} \citep{Kelleher2019,Wohns2022AGenomes}, and \texttt{Relate} \citep{Speidel2019ASamples} can infer genomic genealogies for tens of thousands (\texttt{Relate}) to hundreds of thousands (\texttt{tsinfer}, \texttt{ARG-Needle}) of human samples. \texttt{Relate} and \texttt{tsinfer} can additionally incorporate samples from different time periods and have been used to reconstruct unified genomic genealogies for modern humans and ancient samples of humans, Neanderthals, and Denisovans \citep{Speidel2021InferringGenealogies,Wohns2022AGenomes}. This scalability is facilitated by various statistical simplifications, which result in several limitations in the inferences of these approaches. For example, \texttt{Relate} only reports the marginal trees and not their shared structure, and both \texttt{tsinfer} and \texttt{Relate} only provide point estimates for the tree topologies, which precludes assessments of uncertainty in ARG structure.

So far, most ARG inference development has focused on human and other eukaryotic genomes. However, there are also active efforts to create methods tailored to other types of genomes and systems. For example, \cite{Vaughan2017InferringData} developed a Bayesian approach dubbed \texttt{Bacter},  which is designed to infer ARGs for bacteria based on the ClonalOrigin model \citep{Didelot2010InferenceSequences}. Spurred by the COVID-19 pandemic, \cite{Zhan2023TowardsSARS-CoV-2} recently introduced a method (\texttt{sc2ts}) for ARG reconstruction that can involve millions or more of SARS-CoV-2 genomes. \texttt{sc2ts} is designed to construct and repeatedly update the ARG through time with new samples, which is relevant to ongoing surveillance during pandemics wherein pathogen samples are collected and sequenced in real time.

In summary, there is a burgeoning assortment of methods that enable ARG reconstruction across a range of dataset and system characteristics including data types, sample sizes, sampling regimes. ARG reconstruction remains a substantial statistical and computational challenge, and many improvements in the robustness and flexibility of ARG reconstruction are still needed \citep[e.g.,][]{Deng2021TheGraphs,Brandt2022EvaluationGraphs,Ignatieva2023TheGraphs}. However, ARG inference has emerged as a nexus of methodological development in statistical population genetics and ongoing efforts exist to address the limitations and combine the strengths of existing methods \citep[e.g.,][]{Rasmussen2023Espalier:Forests}. Readers should be prepared for continued innovation in this area.

\subsection{Simulation}
Concurrent with improvements in ARG reconstruction, revolutionary progress in population genomic simulation has occurred over the past decade. One of the most significant developments was \texttt{msprime} \citep{Kelleher2016EfficientSizes,Baumdicker2022Efficient1.0}, which can simulate the genomes and ancestry for a set of samples backwards in time using the coalescent. With the coalescent, only the ancestors of the samples (and not entire populations) need to be tracked. This approach is highly efficient but generally entails an assumption of neutral evolution [although it is possible for coalescent theory and simulation to incorporate selection \citep[e.g., ][]{Kaplan1988TheSelection,Hudson1988TheRecombination.,Walczak2012TheCoalescent,Spencer2004SelSim:Recombination,Kern2016Discoal:Selection,Baumdicker2022Efficient1.0}]. The notable innovation of \texttt{msprime} relative to previous coalescent programs is the speed at which it can perform simulations at biologically realistic scales under a variety of models and with recombination. For example, \texttt{msprime} has been used to simulate realistic whole genome sequences based on genealogical information for $\sim$1.4 million people inhabiting Quebec, Canada \citep{Anderson-Trocme2023OnQuebec}.

Another noteworthy development in population genomic simulation over the past decade is \texttt{SLiM} \citep{Messer2013SLiM:Linkage}. In contrast to coalescent simulators, \texttt{SLiM} simulates forward in time using either Wright-Fisher or non-Wright-Fisher models \citep{Haller2019SLiMModel}. The forward-in-time nature of \texttt{SLiM} means that all individuals in each generation (including historical individuals that are not genetic ancestors to the contemporary population) must be tracked in the simulation. This elevates the computational burden compared to coalescent simulation. However, it enables substantially more flexibility in the scenarios that can be simulated including complex selection and ecological interactions across multiple species \citep{Haller2023SLiMModeling}. Relevant to this review, both \texttt{SLiM} and \texttt{msprime} can record the ARG and/or ARG simplifications during simulation \citep{Haller2019Tree-sequenceGenomes,Baumdicker2022Efficient1.0}. These and other simulation programs [e.g., \texttt{discoal} \citep{Kern2016Discoal:Selection}] can be used for a variety of purposes in ARG-based research including exploration of biological phenomena, statistical and machine learning inference \citep[e.g.,][]{Hejase2022AGraph,Campagna2022SelectiveSpecies,Korfmann2023SimultaneousCoalescent}, and methods evaluation \citep{Brandt2022EvaluationGraphs}.

\subsection{The succinct tree sequence}
The correlated nature of the ARG’s marginal trees can be exploited to compactly encode the trees in a data structure termed the \textit{succinct tree sequence} or \textit{tree sequence} for short \citep[Figure \ref{arg_mutation_fig}A,B;][]{Kelleher2016EfficientSizes,Kelleher2018EfficientSimulation}. The tree sequence defines the trees using two tables. The node table contains an identifier and the timing of each node (first table in Figure \ref{arg_mutation_fig}B). The edge table documents the edges shared between adjoining trees by recording the parent and offspring nodes of each edge and the contiguous extent of the genome that each edge covers (second table in Figure \ref{arg_mutation_fig}B). The key innovation here is that the data structure eliminates substantial redundancy. Instead of storing each tree independently, which would necessitate duplication of shared nodes and edges, the tree sequence records each shared component just once. 

The basic tree sequence technically does not encode the full ARG, which includes all coalescent and recombination events. The basic tree sequence only explicitly contains information on the coalescent events and does not detail the timing and specific changes that differentiate adjacent trees. \cite{Kelleher2019} explain this distinction as follows: the full ARG ``encodes the events that occurred in the history of a sample'' while the set of marginal trees recorded in the tree sequence ``encodes the outcome of those events.'' Nonetheless, the tree sequence can be elaborated with recombination information to completely represent the ARG \citep[e.g.,][]{Baumdicker2022Efficient1.0,Mahmoudi2022BayesianGraphs}.

Several properties of the tree sequence have revolutionized ARG-based research. First, its concise nature means that an immensity of genealogical information can be stored in a highly compressed manner. The tree sequence is also a flexible format that can be augmented with additional tables to store other information such as location metadata and DNA data (e.g., third and fourth tables in Figure \ref{arg_mutation_fig}B; Figure \ref{arg_mutation_fig}A). Notably, relative to conventional genotype matrix formats (Figure \ref{arg_mutation_fig}C), DNA data can be represented much more efficiently using the tree sequence. For instance, \cite{Kelleher2019} estimated that the tree sequence format could store genetic variant data for 10 billion haploid human-like chromosomes in $\sim$1 terabyte, which is many orders of magnitude smaller than the $\sim$25 petabytes required to store these data in a variant call format (VCF) file \citep{Danecek2011}. The efficiency of the tree sequence also permits significant speed-ups in computation (e.g., through the implementation of fast algorithms). These features have enabled advancements in the scale and scope of ARG-based analyses and are increasingly accessible given that the tree sequence underpins a growing ecosystem of methods and software including \texttt{tsinfer}, \texttt{sc2ts}, \texttt{ARGinfer}, \texttt{msprime}, \texttt{SLiM}, and \texttt{tskit} \citep{Kelleher2018EfficientSimulation} built to infer, simulate, and analyze ARGs. Further details on the tree sequence can be found in the papers introducing and expanding the tree sequence \citep{Kelleher2016EfficientSizes,Kelleher2018EfficientSimulation,Mahmoudi2022BayesianGraphs} and in \texttt{tskit}’s documentation (\url{https://tskit.dev/tskit/docs/stable/introduction.html}).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CURRENTLY EXCLUDED TEXT %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Collectively, the existing ARG inference methods can accommodate many of the complications inherent in empirical genomic data. For example, several of the methods (e.g. \texttt{ARGweaver}) are able to handle unphased data by incorporating uncertainty in the phasing into the ARG inference.

%Big takeaway is that there is a growing assortment of methods that enable flexible and accurate ARG reconstruction that is scaleable across a broad range of sample sizes. Hence, available methods can increasingly accommodate the complexities of empirical data.



%Over the past ~decade, revolutionary developments in ARG-based inference, simulation and manipulation.

%List of innovations in ARG reconstructions -- big takeaway is that there is a growing arsenal of methods that enable flexible and accurate ARG reconstruction that is scaleable across a broad range of sample sizes. Hence, available methods can increasingly accommodate the complexities of empirical data.

%\begin{itemize}
%\item Bayesian methods such as ARGweaver, Arbores, and ARGinfer allow for rigorously accounting from uncertainty in the underlying ARG in downstream statistical inferences
%\item Methods like tsinfer/tsdate, Relate/Colate, and ARG-Needle have been explicitly built to handle huge sample sizes---tens of thousands or more
%\item Several methods require phased data, but others do not so available methods can accommodate variation in empirical sequencing data
%\item Colate was designed to include historical samples
%\end{itemize}


%This section is for providing an overview of methodological advancements in ARG-based research. For this, I am thinking about starting with how after the idea of ARGs was proposed, it was largely impractical to actually work with or simulate the ARG and thus it was largely restricted to the theoretical and computational literature (I think this is right?). However, important breakthroughs over the past decade have started to enable the study of ARGs in evolutionary genomics. For this, we could cover developments in ARG inference like bayesian methods such ARGweaver (Rasmussen et al. 2014), Arbores (Heine et al. 2018), and ARGinfer (Mahmoudi et al. 2022), as well as other methods like ARG-Needle (Zhang et al. 2023), tsinfer, tsdate, Relate/Colate (Leo Speidel's stuff), etc. There are other recent methods like Espalier (https://doi.org/10.1101/2022.01.17.476639) and KwARG (https://doi.org/10.1093/bioinformatics/btab351) that also might be worth mentioning. We could also talk about important progress in simulating and storing genomic genealogy information like SLiM, msprime, and tskit, and the succinct tree sequence. Here and/or in the primer section, maybe also talk about how what is is inferred/stored from these methods differs from the true ARG. For example, in addition to discretizing time, ARGweaver uses the sequentially markovian coalescent to computationally simplify their reconstruction of the ARG. However, this entails the assumption that the topologies of the local trees only depend on the previous tree (so trapped ancestral material that isn't found in sample but induces correlations between genomic intervals can't be inferred).

%Maybe also worth discussing how tree sequences can be manipulated and analyzed using other software that has been developed to study data structured as trees (e.g. the ape package in R). Thus, a lot of existing software and approaches could be co-opted to study tree sequences but this will likely require a different toolkit and methods than people have mostly been using to study genomic data. I am thinking that this section could naturally exist as a box in the review, which would allow for more space in the main text to be dedicated to talking about ARG conceptual content and covering the literature.


%Motivated by the extensive sequencing efforts in human genomics, several recently published approaches have been devised with the goal of being scalable to massive genomic datasets. For example, \texttt{ARG-Needle} \citep{Zhang2023Biobank-scaleTraits} and \texttt{tsinfer}/\texttt{tsdate} \citep{Kelleher2019,Wohns2022AGenomes} have inferred genomic genealogies for hundreds to hundreds of thousands of human samples from the UK BioBank \citep{Bycroft2018TheData}, the 1000 Genomes Project \citep{The1000GenomesProjectConsortium2015AConsortium}, and other large databases. \texttt{Relate} \citep{Speidel2019ASamples} can handle a slightly smaller number of genomes (on the scale of tens of thousands) but can incorporate both contemporary and ancient samples \citep{Speidel2021InferringGenealogies}. The scalability of these methods is facilitated by various statistical simplifications, which result in several limitations in the inferences of these approaches. For example, \texttt{Relate} only reports the marginal trees and not their shared structure, and both \texttt{tsinfer} and \texttt{Relate} only provide point estimates for the tree topologies, which precludes assessments of uncertainty in ARG structure. 
%Efforts are ongoing to develop methods that maintain a degree of scalability while addressing some of the inference limitations that feature in existing methods. For example, Rasmussen and Guo (2023) recently introduced a method called \texttt{Espalier} that infers ARGs based on a series of pre-reconstructed, local phylogenies and an approach called maximum agreement forests. \texttt{Espalier} makes inferences about the recombination events separating trees (not just the set of marginal trees estimated by other scalable methods like \texttt{Relate}) while running much faster than \texttt{ARGweaver} (Rasmussen and Guo 2023).

==> sections/NOTINCLUDED_feedback.tex <==
######################
### DATE: 8/7/2023 ###
######################

### NOT ADDRESSED ###
- My biggest-picture comment is that the introduction to the ARG somewhat conflates the stochastic process with the data structure. The focus of Griffiths & Marjoram was on the stochastic process; they introduced a particular way to think about the data structure (just a particular annotation of a pedigree) for that purpose. (Sometimes "ARG" gets used to mean the stochastic process, but I've asked Paul Marjoram, who agrees it shpuld be used to mean the data structure or at least general concept of pedigree-annotated-with-inheritance.)  Section 2.2 is maybe a bit long, so either removing or separating out the (helpful, I think?) intuition arrived at from thinking about the stochastic process might help.

- Before the intro bit that introduces the ARG (top of p.2) perhaps first introduce the pedigree, which has a longer history and everyone is familiar with? (and is not entirely distinct, since people did a lot of annotating pedigrees with how particular maybe-mendelian traits got passed down...) This helps maybe distinguish the various uses of the phrase "ARG" and say which you're talking about (ie coalescent-with-recombination; specific data structure; or a-pedigree-with-some-annotations) ... reading further... I see the pedigree comes up in the main body, but foreshadowing it a bit would be helpful?


- In the middle of p.5 the text starts to conflate the data structure with the stochastic process (ie Hudson's coalescent-with-recombination)

- End of p.5: I'm not looking at Griffiths & Marjoram, but does the GMRCA necessarily exist (for the stochastic process)? Even if it does, it could well be a great deal older than the maximum locus-specific TMRCA, which is (I think?) the oldest time we could hope to infer anything about the ARG from.  (Also, the statement that the ARG stops at the GMRCA is something fairly specifically tied to a particular description of the stochastic process.)

- Is the SPR distance computed on p.9 a labeled SPR distance? (like if two trees had the same topology but different internal nodes at different times, would they have SPR distance zero?)

- If you haven't already, you might be interested in looking at Ralph 2019 TPB, "An empirical approach to demographic inference with genomic data."


### HELPFUL COMMENTS THAT OR MAY NOT NEED TO BE ADDRESSED ###

- You may be interested to see that msprime can flexibly record other types of node now: https://tskit.dev/msprime/docs/latest/ancestry.html#sec-ancestry-additional-nodes



### ADDRESSED ###
- Note that adjacent trees can differ by many SPR moves (not for the continuous-genome stochastic process though).


- The point you're making in the second paragraph of p.10 can also be explained as saying that as you go along the sequence, the top of the tree tends to change faster than the bottom

- Top of p.6: it's a bit more than "an ordered set of genealogical trees along the genome" - you need node labeled trees so you can say which nodes in one tree are the same as certain nodes in the next tree (this is well explained later, but maybe should be said here).

- "For instance, information on unary nodes is difficult or impossible to obtain from contemporary samples." - this isn't actually true in general; I'm working on a paper discussing this (and a method to add back in the unary bits we know something about: https://github.com/tskit-dev/tskit/pull/2651 )- the intuition is that on either side of a coalescent segment we usually know which of the two coalescing segments extend for a bit; in these regions, these are unary nodes.

-A point you (I think?) haven't made is that although usefulness depends on "how well" we can infer the true ARG, it's not clear to what degree we need: a point estimate of the ARG with every individual tree being accurate; or a posterior distribution on the ARG that is sufficiently tightly concentrated about the truth; or a point estimate that differs in many details but shows the right statistical properties (eg the distributions of TMRCAs may be spot on even if many of the individual TMRCAs are not)

- In description of the different types of nodes it might be helpful to provide an additional plain-language interpretation: for instance, you get a node like "R" if a parent who has two children, each of which is the ancestor of a distinct set of samples.

########################################################

==> sections/NOTINCLUDED_notes.tex <==
\section{An ARG primer}
\label{sec:arg_primer}
In the following section, we will incrementally develop an intuition for what ARGs are by starting with the fundamentals of sexual reproduction and genealogical relatedness, which will help clarify how the ARG emerges from these first principles of biology. To simplify our discussion, we will focus on sexual, diploid organisms and meiotic recombination throughout the paper. However, the ideas covered here are relevant to any organism across the tree of life as well as viruses whose genomes undergo any type of recombination (e.g., gene conversion, bacterial conjugation). For more technical treatments of the ARG, we direct interested readers to \cite{Griffiths1997AnGraph}, \cite{Wiuf1999RecombinationSequences}, \cite{Hein2005TheRecombination}, and Wong et al. (YEAR). Although various formulations of the ARG exist, our discussion is consistent with Wong et al.'s (YEAR) genome ARG (gARG).

\subsection{Background}
In sexual, diploid organisms, gametes are generated by the random sampling of a single copy of each chromosome from a diploid cell during meiosis. During reproduction, the parents’ gametes fuse, which leads to a diploid offspring. Thus, the relationships between a set of individuals can be represented by a genealogical pedigree (Figure \ref{arg_review_main_figure_genomearg}A), in which each individual has two parents, from each of whom it has inherited exactly half of its genome. The pedigree consists of nodes, which represent individual organisms, and edges, which connect a subset of the nodes and signify parent-offspring relationships.

By itself, the pedigree can provide coarse estimates of genetic ancestry, such as the expected genetic relatedness between individuals (e.g., 0.50 between full siblings; 0.125 between first cousins), or the expected proportion of the genome inherited from a particular genealogical ancestor. However, from the pedigree alone, we are unable to ascertain the specific chromosomal copy that a parent transmits to their offspring, and thus we are restricted to calculating expected quantities. We could therefore gain more in-depth knowledge of ancestry in the genome by explicitly tracking the transmission of DNA sequences down the pedigree from specific parental to offspring chromosomes.

This discussion of the pedigree highlights multiple key ideas in our build-up to the ARG. First, because each parent contributes only one copy of a particular DNA sequence to its offspring, each copy of the sequence (including copies contained within an individual) experiences its own unique history of inheritance through the pedigree. Second, because a parent only contributes half of its genome to each offspring and not all individuals reproduce, only a subset of the genetic material possessed by historical individuals in the pedigree end up in contemporary individuals. As you travel further back in the pedigree, despite the geometric increase in the number of expected genealogical ancestors [$2^n$ ancestors (assuming no inbreeding) where $n$ equals the number of generations back in time], an increasing proportion of these ancestors contributes no genetic material to their contemporary descendants \citep{Donnelly1983TheDescent,Chang1999RecentIndividuals}. 

If we concentrate on an individual's DNA sequence at a particular locus, we see that each copy of the DNA traverses just one of the manifold possible paths (i.e., series of connected nodes and edges) in the pedigree. The specific pedigree paths through which copies of DNA at a particular locus in contemporary individuals were transmitted from their ancestors represent the genetic genealogy at that locus \citep{Hudson1991GeneProcess,Mathieson2020}. Similar to a pedigree, each edge in the genealogy represents a transmission event of genetic material from parent to offspring. However, in a pedigree, each node is a diploid individual, while in a genetic genealogy, each node represents one of two haploid sequences \textit{within} a diploid individual---the specific chromosome sampled to create a gamete that passes genetic material to the next generation. This genetic genealogy is embedded in the pedigree (Figure \ref{arg_review_main_figure_genomearg}A). The sequence of relationships defined by the pedigree constrains the possible nodes and edges that can exist in the genealogy, but does not fully dictate the identity of these nodes and edges. The genealogy of a locus is determined by both the pedigree structure and the outcome of the gametogenic chromosome sampling at each reproduction event in the pedigree.

The genetic perspective of relatedness is further complicated by another feature of meiosis: recombination. Meiotic recombination, the shuffling of genetic material in the genome during meiosis, occurs via two processes: (1) exchange of genetic material between homologous chromosomes via crossing over during prophase I; (2) random assortment of homologous chromosomes during anaphase I. These recombinational processes can produce a mosaic of genetic ancestry across the haploid genome of the gamete so that a particular gametic genome potentially contains genetic material inherited from different parents both between non-homologous chromosomes and (more commonly) within chromosomes. Recombination therefore results in different histories of inheritance (and thus different genealogies) across the genome, with topological changes to the genealogy associated with recombination breakpoints \citep{Rosenberg2002GenealogicalPolymorphisms}. 

\subsection{The ancestral recombination graph}
The complex web of genetic genealogies across the genome is comprehensively recorded in a graphical structure known as the \textit{ancestral recombination graph} (ARG), which provides complete information regarding the knowable history of inheritance for the genome. Each node in the ARG represents a haploid genome (a \textit{haplotype}) in a real individual that exists now or in the past (Wong et al. YEAR). Each diploid individual therefore contains two haploid genomes and is represented by two nodes. We refer to nodes corresponding to sampled genomes [often, though not necessarily \citep[e.g.,][]{Schaefer2021AnGenomes,Speidel2021InferringGenealogies,Wohns2022AGenomes}, sampled in the present] as \textit{sample nodes} and all other nodes as \textit{nonsample nodes}. If sample nodes have no sampled descendants, they constitute the tips of the ARG. Edges in the ARG indicate paths of inheritance between nodes. The ARG is technically described as a ``directed graph'' because genetic material flows unidirectionally from ancestors to descendants. 

Assuming that sample nodes are sourced from contemporary individuals, the present time in the ARG contains a lineage (i.e., a set of one or more edges connected by nodes forming a continuous path of inheritance) for each sample. Tracing the lineages back in time, some nodes have two edges enter on the future-facing side but only a single outbound edge on the past-facing side (e.g., node \circled{\footnotesize R} in Figure \ref{arg_review_main_figure_genomearg}B). These nodes represent haplotypes in which two lineages merge (or \textit{coalesce}) into a single lineage, which reduces the lineage count by one (the dark gray points in Figure \ref{arg_review_main_figure_genomearg}D). Coalescence occurs when two or more descendent nodes receive (at least part of) their genomes from the same ancestral node \citep{Hein2005TheCoalescent}. From an organismal perspective, these nodes form when a parent provides the same (portion of a) haploid genome to multiple offspring.

Conversely, other nodes have a single edge enter on the future-facing side but two edges exit the past-facing side (e.g., node \circled{\footnotesize Q} in Figure \ref{arg_review_main_figure_genomearg}B), which represents the outcome of recombination \citep{Griffiths1997AnGraph}. Backward in time, the node with two outbound edges on the past-facing side is the recombinant offspring node whose genome is inherited from two parental nodes (e.g., node \circled{\footnotesize C} in Figure \ref{arg_review_main_figure_genomearg}). The two nodes that each receive one of the outbound edges are the parental nodes whose genomes are recombined in the offspring node. For example, in Figure \ref{arg_review_main_figure_genomearg}, \circled{\footnotesize G} and \circled{\footnotesize H} are the parental nodes of \circled{\footnotesize C}. From an organismal perspective, these nodes form when an offspring receives one of its haploid genomes from a parent that represents the outcome of recombination between the parent's two haploid genomes. Recombination splits the genome into separate lineages and thus each portion of the genome experiences a distinct history of inheritance between (traversing the ARG from present to past) the recombination event from which they split to the coalescence event in which they join back up. Consequently, each recombination event increases the number of lineages in the ARG by one (\citealt{Nordborg2001CoalescentTheory}; the red points in Figure \ref{arg_review_main_figure_genomearg}D). One question that may arise here is whether recombination could preclude the lineages from finding common ancestry because it increases the lineage count. However, backwards in time, the lineage count grows via recombination at a linear rate ($kR/2$ where $k$ = lineage count and $R$ = recombination rate) whereas lineages coalesce at a quadratic rate [$k(k -1)/2$], and thus finding common ancestry is guaranteed \citep{Griffiths1997AnGraph}. From a forward-in-time perspective, recombination fuses portions of two parental genomes into a single haplotype (in the recombinant offspring), and thus unites separate lineages into a single lineage. Nodes through which ancestral material is transmitted but are involved in neither coalescence nor recombination of the samples do not determine the topology of the ARG and thus are frequently omitted (we retain several of these nodes in Figure \ref{arg_review_main_figure_genomearg} to highlight the effects of recombination). More generally, nodes that only have one descendant (\textit{unary} nodes) do not directly influence relationships between the sample nodes and thus are often removed via a process called \textit{simplification} \citep{Kelleher2018EfficientSimulation}. 

The ARG records the timing of each node and the portion of the genome that each edge transmits between ancestors and descendants. To trace the genealogy for a particular locus in the genome, you follow the edges through the ARG that contain the focal locus \citep{Griffiths1997AnGraph}. For example, in Figure \ref{arg_review_main_figure_genomearg}B, if you want to extract the genealogy for a locus in the orange segment (between positions 0 and 1) of sample node \circled{\footnotesize B}, you would follow the edges that transmit the orange segment between nodes (i.e., \circled{\footnotesize B} $\rightarrow$ \circled{\footnotesize K} $\rightarrow$ \circled{\footnotesize R} $\rightarrow$ \circled{\footnotesize W} $\rightarrow$ \circled{\footnotesize X}). Eventually, the entire genome finds common ancestry (i.e., all lineages coalesce). The node in which all lineages first coalesce is called the \textit{most recent common ancestor} (MRCA) of the genome or the \textit{Grand MRCA} (GMRCA; \citealt{Griffiths1997AnGraph}). Because all nodes in the ARG trace their ancestry back to this node, the ARG only contains information on ancestral relationships postdating the GMRCA.

The fact that each genomic region bracketed by recombination breakpoints (hereafter \textit{genomic segment}) possesses its own genealogy and that a segment in a single sample node traces only one path back to the MRCA of the entire sample suggests an alternative representation of the ARG: an ordered set of genealogical trees along the genome with labelled sample and nonsample nodes to specify how nodes are shared between trees (\citealt{Griffiths1997AnGraph}; Figure \ref{arg_review_main_figure_genomearg}E). In this tree representation, each genomic segment has its own local (or \textit{marginal}) tree that represents the segment's evolutionary history. If each recombination event occurs at a unique position in the genome, as you shift from one marginal tree to the next (amounting to traversing one recombination breakpoint), the structure of the new tree is identical to its neighbor except for a single edge that is removed and then affixed to a (potentially new) node (Figure \ref{arg_review_main_figure_genomearg}E). In computational parlance, this action is called a \textit{subtree-prune-and-regraft} operation \citep{Song2003OnTrees}. When all recombination events occur at unique locations, the total number of marginal trees will equal one more than the number of recombination events defining the evolutionary relationships in the genome. For example, in Figure \ref{arg_review_main_figure_genomearg}, two recombination events generate three trees. If recombination events occur at the same location (a breakpoint represents $>$1 recombination event), then moving between adjacent trees will involve a corresponding number of subtree-tree-prune-and-regraft operations (one representing each recombination event), and the tree count will be less than one plus the number of recombination events. 

With inclusion of all nodes involved in recombination and coalescence, it is straightforward to switch between the two representations. As previously discussed, the marginal tree for a particular segment can be extracted from the graphical representation of the full ARG by starting at each sample node and tracing the lineages that transmit the segment through the ARG until all lineages meet in the MRCA. Conversely, you can recover the graphical representation of the ARG from the marginal trees by starting with the tree at one end of the set and then sequentially working across the trees, combining the shared nodes and edges, adding the nodes and edges that are not yet included in the graphical structure, and annotating each edge with the genomic segment(s) that it transmits. As a brief illustration, in Figure \ref{arg_review_main_figure_genomearg}E, the first two trees both contain nodes \circled{\footnotesize S} and \circled{\footnotesize Q} with a connecting edge. In the graphical representation, these shared components would be merged and the edge would be annotated with the transmission of the segments between positions 0 and 2 (as shown in Figure \ref{arg_review_main_figure_genomearg}B).

A recombination event can have several consequences for the structure of adjacent trees. First, it could alter the topology (i.e., the specific branching structure) if the new edge joins to a node on a different branch (e.g., the first and second trees in Figure \ref{arg_review_main_figure_genomearg}E). However, if the new edge joins to a different node on the same branch, the topology will remain unchanged, and only the edge lengths (i.e., coalescent times) will be modified (e.g., the second and third trees in Figure \ref{arg_review_main_figure_genomearg}E). It is also possible for the lineage to coalesce back into the same node, which would result in no change to the tree structure. Each marginal tree contains every sample node because all samples possess the entire genome (and thus every segment represented by each tree). However, the collection of nonsample nodes can differ across trees. If the ARG includes all nodes (i.e., every nonsample node is retained), the absence of a node in a marginal tree signals that it does not represent an ancestor for that segment. If the ARG has been simplified (unary nodes removed), the absence of a node either means that it is not an ancestor or that the node does not represent a genome in which coalescence occurred that involved the sample nodes.

There are several key characteristics of the ARG's tree representation. First, the subtree-prune-and-regraft operations that differentiate adjacent trees highlights that nearby trees are generally quite similar and frequently share many nodes and edges \citep{Hudson1991GeneProcess,Rosenberg2002GenealogicalPolymorphisms}. A series of shared nodes and edges between trees indicates that the corresponding genomic segments were found in the same lineage in that portion of the ARG. The correlated nature of the trees can be exploited for highly efficient tree storage and computation (\citealt{Kelleher2016EfficientSizes,Kelleher2018EfficientSimulation}; Figure \ref{arg_mutation_fig}A,B; see Box \ref{box_tree_sequence} for further details). Second, although marginal trees can overlap in structure, a tree can contain components that are not universally found across the entire set of trees (e.g., in Figure \ref{arg_review_main_figure_genomearg}E, node \circled{\footnotesize S} in the first tree is not found in the third tree). The different histories of inheritance mean that each genomic segment may coalesce in different ancestors that potentially existed at different times in the past and that differ from the GMRCA. For example, in Figure \ref{arg_review_main_figure_genomearg}E, node \circled{\footnotesize X} is the MRCA of the first two trees (the same node as the GMRCA) while the third tree's MRCA is node \circled{\footnotesize W}. If the marginal trees' MRCAs existed at different times in the past, this will manifest as variation in tree height \citep{Hudson1991GeneProcess}.

Although the information contained in the graphical and tree representations of the ARG is the same, many readers, especially those with a background in phylogenetics, may prefer to think about ARGs via their tree representations. Unlike the graphical representation, each marginal tree is a familiar object: it is strictly bi- or multi-furcating, meaning that each node has exactly one ancestor and two or more descendants, and that therefore the tree contains no loops (i.e., it is non-reticulate), and is the desired result of a phylogenetic analysis run on a multiple sequence alignment of the DNA in the tree's genomic segment. Building off this intuition, a phylogeneticist may draw on experience and imagine the set of marginal trees as analogous to a Bayesian posterior distribution of phylogenies. However, although this intuition may be useful in getting started with ARGs, it is important to remember that each marginal tree is not independent of the others, both because each is separated from its neighbor by a single recombination event (so is therefore highly correlated), and because the same nodes and edges may appear across multiple marginal trees. The shared structure of trees imbues the nodes and edges with different properties relative to the analogous components in a standard phylogeny. For example, in a standard phylogeny, branches depict ancestor-descendant relationships through time and thus are one-dimensional. In contrast, edges in the ARG exist both through time (extending along the vertical axis in Figure \ref{arg_review_main_figure_genomearg}C) and across the genome (the width along the horizontal axis in Figure \ref{arg_review_main_figure_genomearg}C), and thus can be conceptualized as two-dimensional \citep{Shipilina2022OnBlocks}. The overlapping nature of marginal trees underlies much of the ARG's utility and facilitates the power of ARG-based inference, which we discuss later in the review.























https://tskit.dev/tutorials/args.html#sec-args

potential box ideas and other topics that we may want to talk about:

detailed description of recent methodological developments for inferring, simulating, and working with ARGs. This could also be a section in the main text. 

historical development of the ARG

clarifying terminology about structures that define relatedness. For example, there are several terms that are used with ARGS (at least in this review) including graph, pedigree, genealogy, tree, phylogeny, topology, lineage. What exactly are these things and how are they different from each other?

Another box that could maybe be helpful for people (especially those that have been thinking about phylogenies in a macroevolutionary context is the difference (and similarities) between the tree sequence and phylogenies, gene trees, and other tree-like structures used in macroevolution. 

If we are targeting audience that is largely motivated by a specific organism, maybe we should provide an explicit discussion of what  portion of the tree of life the concept of the ARG applies to? This line of thinking was partially motivated by a general observation that I that I have had about organismal biologists that many times their first question after a lecture is ``does this apply to my study organism?'' This could maybe be a box or maybe fit into the intro or the arg primer section. One question that I have about this is how and whether the ARG is relevant to microbes? This fairly recent genetics paper might be a good place to start thinking about this: https://doi.org/10.1534/genetics.116.193425





The comprehensive nature of the ARG means that it is both highly complex and information rich. These properties can render the ARG unwieldy. However, it also means that the ARG represents a detailed record of evolutionary events and processes that have molded the genomic content of each node. Because evolutionary relationships in the genome are completely encoded in the ARG, it serves as a natural and efficient framework for documenting and summarizing multifarious features of the nodes. Additionally, different evolutionary phenomena regulate the transmission of genetic material in specific ways, and thus each process can leave a particular (and frequently distinct) imprint in the ARG’s structure (i.e. the topology and edge lengths). Mining the ARG for signatures of evolutionary phenomena represents a powerful approach for investigating many topics across evolutionary biology. In this section, we review the ARG's utility for research across multiple major themes in evolutionary biology. For each theme, we include a conceptual background for how relevant information is contained in the ARG and survey the related literature to illustrate how the ARG can enhance empirical research.

The complex web of genetic genealogies across the genome is comprehensively recorded in a graphical structure known as the ancestral recombination graph (ARG), which provides complete information regarding the knowable history of inheritance for the genome. Similar to a genealogical pedigree, time is measured in generations, and each node in the ARG represents a haploid genome in a real individual that exists now or in the past (e.g., each sampled diploid individual consists of two nodes). We refer to nodes corresponding to sampled genomes as \textit{sample nodes} and all other nodes as \textit{nonsample nodes}. If sample nodes have no descendants, they constitute the tips of the ARG. Edges in the ARG indicate paths of inheritance between nodes. The ARG is technically described as a ``directed graph'' because genetic material flows unidirectionally from ancestors to descendants. 

Assuming that sample nodes are sourced from contemporary individuals, the present time in the ARG contains a lineage (i.e., a set of one or more connected edges forming a continuous path of inheritance) for each sample. Tracing the lineages back in time, some nodes have two edges enter on the posterior side (the side facing the present) but only a single outbound edge on the anterior side (e.g. node 6 in Fig. \ref{arg_review_main_figure}B). These nodes represent ancestors in which two lineages merge (or \textit{coalescence}) into a single lineage. Coalescence occurs when a single ancestral node passes the same portion of its genome to two (or more) descendant nodes. Conversely, other nodes have a single edge enter on the posterior side but two edges exit the anterior side (e.g. node C in Fig. \ref{arg_review_main_figure}B), which represents the outcome of recombination. From a backward-in-time perspective, the node with two outbound edges on the anterior side is the recombinant offspring whose genome is inherited from two parents. The two nodes that each receive one of the outbound edges are the parental nodes whose genomes are recombined in the offspring. Recombination splits the genome into separate lineages and thus each portion of the genome experiences a distinct history of inheritance predating recombination (until the lineages coalesce again). Perhaps more intuitively, from a forward-in-time perspective, recombination fuses portions of two parental genomes into a single genome (the recombinant offspring), and thus results in the union of separate lineages into a single lineage. Nodes through which ancestral material is transmitted but are not involved in coalescence or are the product of recombination do not determine the topology of the ARG and are frequently omitted (we retain several of these nodes in Fig. 1 to highlight the effects of recombination). More generally, nodes that only have one descendant (\textit{unary} nodes) do not influence relationships between the sample nodes and thus are often removed via a process termed \textit{simplification} (see Wong et al. YEAR for further details and Fig. SX for how the ARG in Fig 1b would be fully simplified). 


The ARG records the timing of each node and the portion of the genome that each edge transmits between ancestors and descendants. To trace the genealogy for a particular locus in the genome, you follow the edges through the ARG that contain the focal locus. For example, in Fig. 1B, if you want to extract the genealogy for a locus in the orange segment (between positions A and B) of sample node 2, you would follow the edges that transmit the orange segment between nodes (i.e., 2 --> 4 --> 6 --> 7 --> 8). Eventually, the entire genome finds common ancestry (i.e., all lineages coalesce). The node where all lineages first coalesce is termed the \textit{most recent common ancestor} (MRCA) of the genome [or the \textit{Grand MRCA} (GMRCA)]. Because all nodes in the ARG trace their ancestry back to this node, the ARG only contains information on ancestral relationships postdating the GMRCA.

The observations that each genomic region bracketed by recombination breakpoints (hereafter \textit{genomic segment}) possesses a distinct genealogy and that a segment in a single sample node traces only one path back to the MRCA of the entire sample suggests an alternative representation of the ARG. Combined with knowledge of the recombination timing, the edge on which recombination occurred, and the genomic location of the breakpoint, the ARG can equivalently be formulated as a collection of trees along the genome (Fig. \ref{arg_review_main_figure}C). In the tree representation, each genomic segment has its own local (or \textit{marginal}) tree that represents the segment's evolutionary history. If each recombination event occurs at a unique position in the genome, as you shift from one marginal tree to the next (amounting to traversing one recombination breakpoint), the structure of the new tree is identical to its neighbor except for a single edge that is deleted and a new edge that is affixed to a (potentially) new node. In computational parlance, this action is called a \textit{subtree-prune-and-regraft} operation. When all recombination events occur at unique locations, the total number of marginal trees will equal one more than the number of recombination events defining the evolutionary relationships in the genome. For example, in Fig. \ref{arg_review_main_figure}, two recombination events generate three trees. If recombination events occur at the same location (a breakpoint represents $>$1 recombination event), then moving between adjacent trees will involve a corresponding number of subtree-tree-prune-and-regraft operations (one representing each recombination event), and the tree count will be less than one plus the number of recombination events.

A recombination event can have several outcomes on the structure of adjacent trees. First, it could alter the topology (i.e. the specific branching structure) if the new edge joins to a node on a different branch (e.g. the first and second trees in Fig. \ref{arg_review_main_figure}C). However, if the new edge joins to a different node on the same branch, the topology will remain unchanged, and only the edge lengths (i.e. coalescent times) will be modified (e.g. the second and third trees in Fig. \ref{arg_review_main_figure}C). It is also possible for the lineage to coalesce back into the same node, which would result in no change to the tree structure. Each marginal tree contains every sample node because all samples possess the entire the genome (and thus every segment represented by each tree). However, the collection of nonsample nodes can differ across trees. The absence of a node in a marginal tree signals that it does not represent a coalescence node for that segment.
%their histories.

There are several key characteristics of the ARG's tree representation. First, the subtree-prune-and-regraft operations that differentiate adjacent trees highlights that nearby trees are generally highly correlated. Relatedly, trees frequently share many nodes and edges. A series of shared nodes and edges between trees indicates that the corresponding genomic segments were found in the same lineage in that portion of the ARG. The correlated nature of the trees can be leveraged for highly efficient tree storage and computation (see Box \ref{tree_sequence_box} for further details) Second, although marginal trees can overlap in structure, a tree can contain components that are not universally found across the entire set of tree (e.g. in Fig. \ref{arg_review_main_figure}C, node 4 in the first tree is not found in the third tree). The different histories of inheritance mean that each genomic segment may coalesce in different ancestors that potentially existed at different times in the past and that differ from the GMRCA. For example, in Figure \ref{arg_review_main_figure}C, node 8 is the MRCA of the first two trees (the GMRCA) while the third tree's MRCA is node 7. If the marginal trees' MRCAs existed at different times in the past, this will manifest as variation in marginal tree height.














Some additional explanation can help build further intuition regarding the ARG's content and how its structure is created. Different events have contrasting effects on the relationships encoded in the ARG. The particular pattern of coalescence defines the relationships between nodes at a particular locus while recombination alters the relationships across different portions of the genome. Nodes through which ancestral material is transmitted but are not involved in coalescence or the product of recombination do not determine the topology of the ARG and are frequently omitted (we retain several of these nodes in Fig. 1 to highlight the effects of recombination). More generally, nodes that only have one descendant (\textit{unary} nodes) do not influence relationships between the sample nodes and thus are often removed via a process termed \textit{simplification} (see Wong et al. YEAR for further details and Fig. SX for how the ARG in Fig 1b would be fully simplified). 
The nodes in the ARG represent only a subset of the genetic material possessed by individuals in the pedigree. This filtering phenomenon occurs for two reasons. First, as previously mentioned, the genomes of contemporary individuals were transmitted through only a subset of chromosomes found in the pedigree. Logically, the historical chromosomes that are not genetic ancestors will not appear in the ARG. Additionally, the breakpoints reflected in the ARG only represent the recombination events that determine the evolutionary relationships of the sample nodes. Myriad recombination events may have transpired in the ancestors found in the pedigree and may involve the genomes represented by the nonsample nodes in the ARG. However, if a recombination event takes place in part of a nonsample node's genome that is not inherited by the sample nodes (e.g. sample nodes inherit a nonsample node's genome between positions 0--5000 but the recombination breakpoint is at 10000/10001), then those events will not be recorded in the ARG.






Second, based on our discussion, the ARG only includes nodes that define the structure of the genetic genealogies via coalescence and recombination (that is, nodes at which lineages being traced backward in time meet or diverge). Ancestral chromosomes from which samples inherit genetic material but that do not determine relationships between samples (\textit{unary} nodes) are generally omitted from the ARG (shown as dashed circles in Fig. \ref{arg_review_main_figure}B). Additionally, the breakpoints reflected in the ARG only represent the recombination events that determine the evolutionary relationships of the sample nodes. Myriad recombination events may have transpired in the ancestors found in the pedigree and may involve the nonsample nodes in the ARG. However, if a recombination event takes place in part of a nonsample node's genome that is not inherited by the sample nodes (e.g. sample nodes inherit a nonsample node's genome between positions 0--5000 but the recombination breakpoint is at 10000/10001), then those events will not be recorded in the ARG.



%For example, in Figure X, crossing over between homologous chromosomes leads to part of a chromosome arm associated with the maternal homolog and the remainder of the chromosome associated with the paternal homolog. The recombination event would result in two distinct histories (that is, distinct genealogies) for that chromosome---one associated with the maternal portion and the other associated with the paternal portion. 


Griffiths and Marjoram (1997) original formulation, the ARG is the stochastic outcome of a coalescent process involving recombination. In this view, 


How do the stochastic process and data structure perspectives differ? The stochastic process is governed by a particular model of coalescence with recombination, and thus the ARG displays properties associated with this model. For example, the timing of coalescence and recombination events are governed by particular probability distributions of waiting times. 

In contrast, the ARG as a data structure is a broader perspective that simply depicts how genetic material is transmitted down a pedigree when reproduction involves recombination. The ARG is not governed by any particular model, and it does not necessarily show any properties associated with the coalescent.

Nonetheless, despite our knowledge regarding empirical limits on ARG reconstruction, it remains unclear the degree of accuracy needed to make quality downstream inferences that derive from the ARG. For example, do accurate inferences generally require ARGs with correct marginal trees topologies? Or perhaps some questions only require certain properties of the ARG to be accurate. For example, the distribution of TMRCAs may need to be accurate while the accuracy of marginal topologies is less crucial. Understanding the sensitivities and requirements of downstream inferences will help uncover the particular facet(s) of ARG reconstruction in most need of improvement and will also help delineate the limits that empirical ARG reconstruction places on downstream inferences.










%from the Wong paper
%Thus we can think of an ARG as being any structure that encodes the reticulate genetic ancestry of a sample of colinear sequences under 505 the influence of recombination.



